Baryonification extended to thermal Sunyaev Zeldovich

Baryonification algorithms model the impact of galaxy formation and feedback on the matter field in gravity-only simulations by adopting physically motivated parametric prescriptions. In this paper, we extend these models to describe gas temperature and pressure, allowing for a self-consistent modelling of the thermal Sunyaev-Zeldovich effect, weak gravitational lensing, and their cross-correlation, down to small scales. We validate our approach by showing that it can simultaneously reproduce the electron pressure, gas, stellar, and dark matter power spectra as measured in all BAHAMAS hydrodynamical simulations. Specifically, with only two additional free parameters, we can fit the electron pressure auto- and cross-power spectra at 10% while reproducing the suppression in the matter power spectrum induced by baryons at the per cent level, for different AGN feedback strengths in BAHAMAS. Furthermore, we reproduce BAHAMAS convergence and thermal Sunyaev Zeldovich angular power spectra within 1% and 10% accuracy, respectively, down to l = 5000. When used jointly with cosmological rescaling algorithms, the baryonification presented here will allow a fast and accurate exploration of cosmological and astrophysical scenarios. Therefore, it can be employed to create mock catalogues, lightcones, and large training sets for emulators aimed at interpreting forthcoming multi-wavelength observations of the large-scale structure of the Universe.

==> commented.tex <==
\mycomment{
\noindent When using the bound gas density profile of \cite{Martizzi2013,Schneider&Teyssier2015,Arico2020},   
\begin{equation}
\rho_{\rm BG} (x) = y_0 \left[ \frac{\ln (1+x)}{x}  \right]^{\frac{1}{\Gamma-1}},
\end{equation}
where $x=r/r_{\rm s}$, $r_{\rm s}$ is the NFW scale radius, then 
 $x'=\sqrt5 c$. 
For the ejected gas, we consider the following parametrisation:
\begin{equation}
T_{ej} = T_{\rm AGN} \cdot 10^{m_{\rm AGN} \cdot [\log (M_{\rm g}/(10^8 M_{\odot} h^{-1}))]},
\label{eq:T_agn}
\end{equation}
%where $M_{\rm g}$ is the central galaxy mass, and $T_{\rm AGN}$ and $m_{\rm AGN}$ are free parameters. As shown in Fig.\ref{fig:T_agn}, they control the amplitude and slope of the ejected temperature with respect to the host galaxy mass, respectively. We assume the temperature of the ejected gas to be constant with radii, but dependent on the host galaxy mass. This could be understood qualitatively by the fact that larger galaxies host larger super massive black holes, and their haloes are massive enough to retain most of the gas. These results in higher gas temperatures, although the deep gravitational potential does not allow the gas to escape the halo. For $T_{\rm AGN} = 10^{5} \, K$ and $m_{\rm AGN} = 0.7$, we recover roughly the same dependence found in Illustris TNG \citep{Nelson2019}, and therefore we fix these values in the rest of the paper.
\begin{figure}
\includegraphics[width=.48\textwidth]{figs/T_agn.png}
\caption{Temperature of the expelled gas as a function of the host galaxy mass, 
varying the parameter $T_{\rm AGN}$ (upper panel) and $m_{\rm AGN}$(lower panel).}
\label{fig:T_agn}
\end{figure}
}



\mycomment{
\begin{equation}
P_{\rm BG}^{\rm nth} (r) = P_0^{\rm nth}  \cdot \rho_{\rm BG} (r) ^{\Gamma^{\rm nth}}.
\end{equation}

Rather than consider the unknown $P_0^{\rm nth}$ and $\Gamma^{\rm nth}$ as free parameters, we parametrise the ratio with respect to the amplitude and index of the total pressure, $\alpha^{nth}=P_0^{\rm nth}/P_0$ and $\beta^{\rm nth}=\Gamma^{\rm nth}/\Gamma$. Thus, the temperature profile now reads 

\begin{equation}
T_{\rm BG} (r) = T_0 \cdot  \rho_{\rm BG} (r) ^{\Gamma-1} \left[  1 - \alpha_{\rm nth} \rho_{\rm BG} (r) ^{\Gamma (\beta_{\rm nth}-1)}  \right].
\end{equation}
Note that for $\alpha^{nth}=0$ we assume a negligible non-thermal contribution to pressure, and therefore we recover Eq.\ref{eq:temp_1}. If $\beta^{nth}=0$ the non-thermal pressure is assumed radially constant. In the case where $\beta^{nth}=1$, the thermal and non-thermal contributions have the same radial dependence. In this last case, the hydrostatic mass bias, defined as $(1-b_{\rm h}) \equiv M^{th}/M^{tot}$, is simply $b_{\rm h} = \alpha_{\rm nth}$. 
}




\subsection{Thermodynamical profiles}

\begin{figure*}
\centering
\includegraphics[width=.49\textwidth]{figs/density_nenya.pdf}
\includegraphics[width=.49\textwidth]{figs/temperature_nenya.pdf}
\caption{Density field in a baryonified simulation, weighted by gas mass (left panel) and temperature (right panel). The BCM parameters have been tuned to generate relatively strong AGN feedback.}
\label{fig:bar_fields}
\end{figure*}

To predict the main thermodynamical properties of gas particles, we parameterise the halo gas temperature and pressure profiles, and then we assign to each particle a given temperature and pressure, according to its radial distance from the halo centres. We assume a polytropic equation of state of the gas, where the temperature and pressure are given by the polytropic index $\Gamma$. Finally, we use the same gas density profile in haloes as \cite{Arico2020b}, i.e. 

\begin{equation}
\rho_{\rm BG}(r\le r_{\rm out}) = \rho_0 \frac{1}{ (1+r/r_{\rm inn})^{\beta_{i}} } \frac{1}{(1+(r/r_{\rm out})^2)^2}
\label{eq:rho_bg}
\end{equation}

\noindent where $\rho_0$ is a normalisation factor,  $r_{\rm inn}$ and $r_{\rm out}$ define where the slope changes at small and large radii, respectively. We define the inner radius $r_{\rm inn}=\theta_{\rm inn} \times r_{200}$ and outer radius $r_{\rm out}=\theta_{\rm out} \times r_{200}$, beyond which the gas profile perfectly traces the dark matter, i.e. a Navarro-Frenk-White (NFW) profile \citep{NFW1997}. The gas inner slope depends on halo mass as $\beta_{i}=3-(M_{\rm inn}/M_{200})^{\mu_{i}}$. $\theta_{\rm inn}$, $\theta_{\rm out}$, $M_{\rm inn}$ and $\mu_{i}$ are free parameters. 

The polytropic temperature profile is 
\begin{equation}
T_{\rm BG} (r) = T_0 \times  \rho_{\rm BG} (r) ^{\Gamma-1};
\label{eq:temp_1}
\end{equation}
where 
\begin{equation}
T_0 = \frac{4 \pi G \rho_{\rm s} r_{\rm s}^{2}}{\rho_0^{\Gamma-1}} \frac{\mu m_{\rm p}}{k_{\rm B}} \frac{\Gamma -1}{\Gamma}.
\end{equation}
with $G$ the gravitational constant, $\rho_{\rm s}$ the dark matter density at $r_{\rm s}$, $m_{\rm p}$ is the proton mass, and $k_{\rm B}$ is the Boltzmann constant. We assume for simplicity a fully ionised gas composed of $X=76\%$ hydrogen and $Y=24\%$ helium. Thus, in our case, the mean molecular weight is simply $\mu = 4/(5X+3) \approx 0.59$. We note that we could in principle use more complicated models, with metals and partial ionisation levels, but they would likely not affect our results at a significant level. 

In this work, we model the polytropic index as 

\begin{equation}
\Gamma = 1 + \frac{(1+x')\ln(1+x')-x'}{(1+3x')\ln(1+x')},
\end{equation}

 \noindent where $x'= c \times \theta_{\rm out}$ and $c$ is the halo concentration \citep[see e.g.][]{Martizzi2013,Schneider&Teyssier2015,Arico2020}. Another possible approach is to fit directly the polytropic index to the data. 

By imposing the ideal gas law, the pressure profile is simply

\begin{equation}
P_{\rm BG} (r) =  \rho_{\rm BG} \frac{k_{\rm B} T_{\rm BG}}{\mu m_p}.
\label{eq:press_1}
\end{equation}

For simplicity, we assume that the gas ejected from the haloes by feedback has the same temperature profile as the bound gas, i.e. it thermalises instantaneously. We note that the ejected gas component features a small mass fraction and low density, thus its contribution to the tSZ is expected to be subdominant even if heated at high temperatures. 

In Fig. \ref{fig:bound_profiles} we show an example of the density, temperature, and pressure profiles in haloes of mass comprised between $10^{12} \, {\it h}^{-1} M_{\odot}$ and $10^{15} \, {\it h}^{-1} M_{\odot}$, considering the best-fitting parameters to the matter power spectrum of the BAHAMAS simulation \citep{McCarthy2017}. For reference, we over-plot the virial temperature and the universal pressure profiles from \cite{Arnaud2010} as dashed lines. We observe that $T_0$ is very close to the virial temperature and $P_{\rm BG}$ to the universal profiles, especially for massive haloes. We remind the reader that the universal pressure profiles have been fitted to haloes of $M \ge 10^{14} \, \Msun$, which contribute the most to the tSZ signal.

\subsection{Non-thermal pressure}
So far, we have assumed that the gas in hydrostatic equilibrium within haloes is solely supported by thermal pressure. In reality, hydrodynamical simulations and (indirect) observations have shown that a given amount of non-thermal pressure is expected \citep{Shaw2010,Hurier2018,Akino2022}. Taking it into account through the so-called hydrostatic mass bias, it is possible to reconcile the total mass of the clusters obtained with "direct" measurements (i.e. weak lensing) with the ones inferred assuming hydrostatic equilibrium from e.g. X-ray or microwave observations. The hydrostatic mass bias is related to the non-thermal pressure support not accounted for, arguably produced by turbulence, cosmic rays, and magnetic fields \citep{Green2020,Ettori&Eckert2022}. 

The non-thermal contribution can be as high as 50\% of the total pressure in the outskirt of the haloes, and therefore impacts significantly tSZ predictions. In particular, \cite{Green2020} have studied the non-thermal contribution using analytical total pressure profiles \citep{Komatsu&Seljak2001}, non-thermal contribution driven by halo mass assembly \citep{Shi&Kmoatsu2014}, and models for the mass assembly histories \citep{Parkinson2008,vandenBosch2014}. They find that the non-thermal term is roughly universal when expressed as a function of peak height, and they compare their results against hydrodynamical simulations finding a good agreement. 

In this work, we use the fitting function by \cite{Green2020} to model the non-thermal contribution to pressure (and temperature). The thermal pressure and temperature are, respectively,  
\begin{equation}
P_{\rm BG, th}(r) = f_{\rm th}(r/r_{\rm 200m}) \, P_{\rm BG} (r),
\end{equation}
and  
\begin{equation}
T_{\rm BG, th}(r) = f_{\rm th}(r/r_{\rm 200m}) \, T_{\rm BG} (r),
\end{equation}
where
\begin{equation}
f_{\rm th} (x) = A \left( 1 + e^{-(x/B)^C} \right)  \left( \nu/4.1 \right)^{D / (1+[x/E]^F) }, 
\end{equation}
with the radii $x=r/r_{\rm 200m}$ and peak height $\nu=\nu_{\rm 200m}$ are referred to spheres where the mean density is 200 times larger than the mean matter density of the universe. The best-fitting values of the parameters are $A=0.495$, $B=0.719$, $C=1.417$, $D=-0.166$, $E=0.265$, and $F=-2.116$. We show in Fig. \ref{fig:bound_profiles} the thermal contribution to the total pressure with dotted lines. 

We will employ the parametrisation 
\begin{equation}
A = A_{\rm nth} (1+z)^{\alpha_{\rm nth}}
\end{equation}
with $A_{\rm nth}$ and $\alpha_{\rm nth}$ to model possible residual dependence on the amplitude and redshift of the non-thermal contribution, leaving the radial dependence unaltered. 

\raul{explain a bit better}

